Graph Neural Networks with Learnable and Optimal Polynomial Bases

Polynomial filters, a kind of Graph Neural Networks, typically use a predetermined polynomial basis and learn the coefficients from the training data. It has been observed that the effectiveness of the model is highly dependent on the property of the polynomial basis. Consequently, two natural and fundamental questions arise: Can we learn a suitable polynomial basis from the training data? Can we determine the optimal polynomial basis for a given graph and node features? In this paper, we propose two spectral GNN models that provide positive answers to the questions posed above. First, inspired by Favard's Theorem, we propose the FavardGNN model, which learns a polynomial basis from the space of all possible orthonormal bases. Second, we examine the supposedly unsolvable definition of optimal polynomial basis from Wang & Zhang (2022) and propose a simple model, OptBasisGNN, which computes the optimal basis for a given graph structure and graph signal. Extensive experiments are conducted to demonstrate the effectiveness of our proposed models. Our code is available at https://github.com/yuziGuo/FarOptBasis.

==> algorithms/next_basis.tex <==
\begin{algorithm}[tb]
    \SetAlgoNoLine
    \KwIn{
        Normalized graph adjacency $\hat{P}$; 
        Solved basis vectors $v_0, \cdots, v_k$ ($k \geq 0$)
    }
    \KwOut{$v_{k + 1}$} 
    \BlankLine
    \Indp
    % \Foreach{channel \in $X$}{}
    Step $1$: $v_{k + 1}^{\ast} \leftarrow \hat{P} v_k$
    \\
    Step $2$: 
    $
    v_{k + 1}^{\bot} \leftarrow v_{k + 1}^{\ast} -
      \sum_{i=0}^{k}\langle v_{k + 1}^{\ast}, v_i \rangle v_i 
      $
    \\
    Step $3$: $v_{k + 1} \leftarrow v_{k + 1}^{\bot} / \| v_{k +
      1}^{\bot} \|$
    \\
    \KwRet{$v_{k + 1}$}
    \caption{\textsc{ObtainNextBasisVector (Raw Version)}}
    \label{alg:nextbasis_raw}
\end{algorithm}

==> algorithms/next_basis_improved.tex <==
\begin{algorithm}[t]
    \SetAlgoNoLine
    \KwIn{
        Normalized graph $\hat{P}$; 
        \textbf{Two} solved basis vectors $v_{k - 1}, v_k$ ($k \geq 0$)
    }
    \KwOut{$v_{k + 1}$} 
    \BlankLine
    \Indp
    % \Foreach{channel \in $X$}{}
    Step $1$: $v_{k + 1}^{\ast} \leftarrow \hat{P} v_k$
    \\
    Step $2$: $v_{k + 1}^{\bot} \leftarrow v_{k + 1}^{\ast} - \langle v_{k + 1}^{\ast}, v_k \rangle v_k - \langle v_{k + 1}^{\ast}, v_{k - 1}\rangle v_{k-1}$
    \\
    Step $3$: $v_{k + 1} \leftarrow v_{k + 1}^{\bot} / \| v_{k +
      1}^{\bot} \|$
    \\
    \KwRet{$v_{k + 1}$}
    \caption{\textsc{ObtainNextBasisVector}}
    \label{alg:nextbasis_improved}
\end{algorithm}

==> chapters/Motivation.tex <==
\begin{figure*}
   \centering
   \includegraphics[width=2\columnwidth]{images/example.pdf}
   \caption{Representation of $h(\lambda)=\lambda^2 + 1$ by 
      different bases.}
   \label{fig:example}
\end{figure*}

% \section{Motivation and Contribution}
\section{Introduction}


\paragraph{Two Questions.}
Up to now, several bases have been chosen to better approximate the ideal polynomial.
However, there remain two open problems.

\textbf{Question 1: }
Up to now, the works that learn filters use \textit{learnable} coefficients 
above \textit{fixed} polynomial bases, 
and these different bases show different empirical performances.  
Now that the choice of basis matters, 
and the proportion of polynomial bases that we can name it is small,    
\textbf{can we learn polynomial bases from a wide range}? 
One step further, 
to avoid the mutual influence of basis polynomials and the influence of lens, 
we ask: can we learn arbitrary rational \textbf{orthonormal} polynomial bases?
\footnote{For the concrete definition of orthonormal polynomial bases, 
please check the preliminaries in Section \ref{para:inner_product}.}

\textbf{Question 2: }
On the other hand, although these bases differ in empirical performances, 
from the angle of representation ability, they should be the same: 
Any target polynomial of order $K$ can be represented by 
any complete polynomial basis with truncated order $K$. 
% Figure \ref{fig:example} shows an example.
Then, where does the difference in empirical performances come from? 
\textbf{Is there a criterion for an only optimal basis? 
Can we solve this optimal basis?}


% \input{submodules/QuestionToWang.tex}

\subsection{Our Contributions.}


==> submodules/QuestionToWang.tex <==
\subsection{Our questions to Wang's work}

We continue the definition of optimal basis, and raise two questions:

The first question: is there a {\textbf{wider range}} of orthonormal basis
to choose from?

The second question: the {\textbf{optimal}} basis is actually already given by
Wang et al. {\textbf{Can we use this optimal basis without solving its weight
function?}}

Luckily, the answer of both is true.

==> submodules/three_term_briefly.tex <==
% \textbf{Three-Term Recurrences.\quad} 
The fact of three-term recurrences is 
one of the most characteristic features of orthogonal polynomials~\cite{Chihara1990threeterm}, and has been used for multiple times 
in the context of current spectral GNNs. 
The Theorem states that, every sequence of orthogonal polynomials satisfies a three-term recurrence relation of a very special form, that is, 
the polynomial of order $k + 1$ $(k > 1)$ can be expressed by the polynomial of order $k$ and
order $k - 1$:

\input{theorems/forms/3_term_general.tex}

% In the context of polynomial filtering, 
% the three-term recurrences in fact have been used multiple times. 
In polynomial filters, such recurrence relation permits the calculation of $g_{k+1}(\hat{P})x$ to reuse $g_k(\hat{P})x$ and $g_{k-1}(\hat{P})x$. 
\cite{Defferrard2016cheb} 
owe the fast filtering of ChebNet to employing the three-term recurrences of \textbf{Chebyshev polynomials} (the first kind, 
which is orthogonal w.r.t.  $\frac{1}{\sqrt{x^2-1}}$): 
$T_{k+1}(x) = 2xT_k(x)-T_{k-1}(x)$. 
Similarly, 
JacobiConv\cite{Wang2022jacobi} employs the 
three-term recurrences for \textbf{Jacobi polynomials} (orthogonal w.r.t. to $(1-x)^{\alpha}(1+x)^{\beta}$). 
Both the Chebyshev basis and Jacobi basis are well-known classic orthogonal polynomials with simple weight functions, 
but from the three-term recurrence relations, 
% of whom we state the complete theorem with proof in Appendix \ref{sec:proof-of-3term},
we know that \textbf{all} the orthogonal polynomial series satisfy, and thus can benefit from such a formula. 

% \textbf{Favard's Theorem.\quad}
Notably, there is a \textbf{converse} theorem of the three-term recurrences: 
Favard's Theorem~\cite{favard1935polynomes}. 
% Please check Appendix \ref{sec:favard-monomial}
% for the complete form of Favard's Theorem, 
% and Appendix \ref{sec:proof-of-far} 
% for the extension of Favard's Theorem to general orthogonal polynomials. 
Please check Appendix \ref{sec:proof-of-3term}, \ref{sec:favard-monomial} and \ref{sec:proof-of-far} for \textcolor{blue}{the proof of} three-term recurrences and a more formal state of Favard's Theorem. 


==> tables/filter.tex <==
\begin{table*}[htp]
    \centering
    \tiny
    \caption{Illustration of our multichannel filter learing experiment.}
    \vskip 0.01in
    % \abovespace
    % \specialrule{0.01in}{0.01in}
    \begin{tabular}
      {p{3.1cm}p{3.2cm}p{3.2cm}p{3.2cm}p{3.1cm}}
      \hline
      Original Image & Y: Band reject
      
      Cb: low pass
      
      Cr: high pass & Y: high pass
      
      Cb: high pass
      
      Cr: low pass & Y: high pass
      
      Cb: low pass
      
      Cr: high pass & Y: low pass
      
      Cb: band reject
      
      Cr: band reject\\
      \hline
      \raisebox{0.0\height}{\includegraphics[width=3.2cm,height=3.2cm]{figures/icml-1.pdf}}
      &
      \raisebox{0.0\height}{\includegraphics[width=3.2cm,height=3.2cm]{figures/icml-2.pdf}}
      &
      \raisebox{0.0\height}{\includegraphics[width=3.2cm,height=3.2cm]{figures/icml-3.pdf}}
      &
      \raisebox{0.0\height}{\includegraphics[width=3.2cm,height=3.2cm]{figures/icml-4.pdf}}
      &
      \raisebox{0.0\height}{\includegraphics[width=3.2cm,height=3.2cm]{figures/icml-5.pdf}}\\
      \hline
    \end{tabular}
    \label{tbl:filtering}
  \end{table*}

==> tables/filters.tex <==
\begin{table}[bp]
    % \small
    \caption{Filters. }
    \label{tbl:filters}
    \begin{tabularx}{1.0\columnwidth}
      % \label{tbl:notations}
      {lXX}
        \toprule
        {\tmstrong{Model}} & {\tmstrong{$h^{\ast}(\hat{L})$}} &  {\tmstrong{$h(\hat{L})$}} \\
        \hline
        % \multicolumn{3}{c}{Fixed Filtered} \\
        % \hline
        GCN & $ I-\hat{L}$ &  $I-\hat{L}$ 
        \\
        APPNP & $ (I - (1-\alpha)(\hat{P}))^{-1} $   & 
        \\
        GNN-LF & &
        \\

        \bottomrule
      \end{tabularx}
    \end{table}

==> tables/learn_filters.tex <==
\begin{table*}[htp]
    \tiny
    \centering
    \caption{Learning process with different basis with {\textbf{one}} image.}
    \begin{tabular}{|p{8.0cm}p{8.0cm}|}
      \hline
      {\textbf{Y}}: Band reject; {\textbf{Cb}}: low pass; {\textbf{Cr}}:
      high pass & {\textbf{Y}}: high pass; {\textbf{Cb}}: high pass;
      {\textbf{Cr}}: low pass\\
      \raisebox{0.0\height}{\includegraphics[width=8.0cm,height=6.062639380821199cm]{figures/icml-6.pdf}}
      &
      \raisebox{0.0\height}{\includegraphics[width=8.0cm,height=6.124458874458875cm]{figures/icml-7.pdf}}\\
      {\textbf{Y}}: high pass; {\textbf{Cb}}: low pass; {\textbf{Cr}}:
      high pass & {\textbf{Y}}: low pass; {\textbf{Cb}}: band reject;
      {\textbf{Cr}}: band reject\\
      \raisebox{0.0\height}{\includegraphics[width=8.0cm,height=6.055243998425817cm]{figures/icml-8.pdf}}
      &
      \raisebox{0.0\height}{\includegraphics[width=8.0cm,height=6.06477108749836cm]{figures/icml-9.pdf}}\\
      \hline
    \end{tabular}
    \label{tbl:learn_filtering}
  \end{table*}
  

==> tables/semi.tex <==
\begin{table}[h]
    \caption{\#Training Nodes \tmcolor{blue}{per class}.}
    \begin{tabular}{|lllll|}
      \hline
      Train/Val/Test Split & 2.5/2.5/95 & {\textbf{10/10/80}} & 20/20/60 &
      60/20/20\\
      \hline
      Citeseer (3,327) & 14 & 55 & 110 & 330\\
      Squirrel (5,201) & 32 & 130 & 260 & 780\\
      \hline
    \end{tabular}
    \label{tbl:semi}
\end{table}

==> theorems/forms/3_term_general.tex <==
% \begin{align*}
%     \label{eq:formula_orthogonal}
% % \[
%     & p_{k + 1} (x) = (A_k x + B_k) p_k (x) + C_k p_{k - 1} (x), \notag \\
%     & p_{-1}(x) \assign 0,  
%     % \notag \\
%     A_k, C_k \in \mathbb{R}^{+}, \ B_k \in \mathbb{R}, \  k \geq 0.    
% \end{align*} 
$\quad p_{k + 1} (x) = (A_k x + B_k) p_k (x) + C_k p_{k - 1} (x)$,

$\quad p_{-1}(x) \assign 0,  
    A_k, C_k \in \mathbb{R}^{+}, \ B_k \in \mathbb{R}, \  k \geq 0.$

==> theorems/forms/3_term_implicit_poly.tex <==
\begin{align*}
    \label{eq:formula_implicit_poly}
    { {\|v^{\bot}_{k+1}\|} }  & g_{k + 1} (\mu) 
      = ( \mu - \langle v_{k + 1}^{\ast},  v_k \rangle) g_k (\mu) 
     \notag  \\
    &\quad\quad\quad - {{\|v^{\bot}_{k}\|}} g_{k - 1} (\mu), 
    \notag \\
     & g_{-1}(\mu) \assign 0, \ g_0 (\mu)  = 1 / \|x\|,
      \notag \\ 
     & k = 0,\cdots,K-1 .
\end{align*}
